Lightweight and Post-Training Structured Pruning for On-Device Large Lanaguage Models

Considering the hardware-friendly characteristics and broad applicability, structured pruning has emerged as an efficient solution to reduce the resource demands of large language models (LLMs) on resource-constrained devices. Traditional structured pruning methods often need fine-tuning to recover performance loss, which incurs high memory overhead and substantial data requirements, rendering them unsuitable for on-device applications. Additionally, post-training structured pruning techniques typically necessitate specific activation functions or architectural modifications, thereby limiting their scope of applications. Herein, we introduce COMP, a lightweight post-training structured pruning method that employs a hybrid-granularity pruning strategy. COMP initially prunes selected model layers based on their importance at a coarse granularity, followed by fine-grained neuron pruning within the dense layers of each remaining model layer. To more accurately evaluate neuron importance, COMP introduces a new matrix condition-based metric. Subsequently, COMP utilizes mask tuning to recover accuracy without the need for fine-tuning, significantly reducing memory consumption. Experimental results demonstrate that COMP improves performance by 6.13\% on the LLaMA-2-7B model with a 20\% pruning ratio compared to LLM-Pruner, while simultaneously reducing memory overhead by 80\%.

==> contents/backup/intro_backup012201.tex <==
%Large language models (LLMs) have demonstrated remarkable versatility and success in various practical applications, including %dialogue systems \cite{yi2024survey}, question answering \cite{zhuang2023toolqa}, and text summarization %\cite{jin2024comprehensive}.
Large language models (LLMs) have demonstrated remarkable success in various practical applications \cite{yi2024survey, zhuang2023toolqa, jin2024comprehensive}. 
The exceptional performance is primarily attributed to their immense number of parameters. 
However, LLMs always require substantial computing power and memory capacity for effective and efficient inference \cite{lin2024exploding, patterson2021carbon}, which severely impedes deployment on resource-constrained hardware, such as edge modules for autonomous vehicles \cite{cui2024drive} or mobile platforms \cite{yin2024llm}.
% , leading to critical challenges in terms of computing power, memory capacity, and inference latency \cite{lin2024exploding, patterson2021carbon}.
To address these concerns, model compression has gained considerable attention to reduce resource footprint and/or accelerate inference speed of LLMs \cite{brown2020language, strubell2020energy}.

%Model pruning is a widely recognized technique for compressing models by selectively removing parameters that contribute minimally to overall performance. 
As one of the dominant model compression techniques, model pruning is widely used and can be categorized into unstructured pruning, structured pruning, and semi-structured pruning.  
Concretely, unstructured pruning is permitted to remove any individual weights (\ie, connections) of a model without adhering to any predefined structure (\eg, neurons, attention heads) \cite{han2015learning, frankle2018lottery, frankle2019stabilizing}, and semi-structured pruning typically removes groups of weights that adhere to certain structural constraints, such as 2:4 (2 out of every 4 consecutive weights are selected and pruned) or 4:8 \cite{frantar2023sparsegpt, zhang2024plug}.
As the removed weights are set to zero, the resulting sparse weight matrices necessitate specialized hardware, \eg, NVIDIA Ampere GPUs \cite{choquette2021nvidia}, for sparse operations, potentially limiting the applicability of both unstructured and semi-structured pruning.
In contrast, structured pruning directly removes structural components such as neurons, attention heads, or entire layers \cite{kwon2022fast, zhang2024loraprune, men2024shortgpt}. %加些参考文献
This makes structured pruning more computationally efficient and less dependent on specialized hardware for performance gains, facilitating broader applicability across various hardware platforms.

Given its hardware-friendly nature, we opt to implement structured pruning on ubiquitous and resource-constrained devices.
However, existing structured pruning methods still encounter two major drawbacks.
% One is high memory consumption, mainly coming from the gradient-based evaluation of \rednote{module} importance.
First, the gradient-based evaluation of module importance will result in excessive memory overhead. 
% For example, LLM-Pruner \cite{ma2023llmpruner} consumes over 32GB of memory to evaluate \rednote{group} importance when pruning a 7B model, making the process highly memory-intensive. 
For example, LLM-Pruner \cite{ma2023llmpruner} requires over 32GB of memory to compute group importance when pruning a 7B model, making the process particularly resource-intensive.
% The other is accuracy loss. 
% As structured pruning explicitly removes entire components from the model, it will lead to larger accuracy loss compared to unstructured pruning given the same pruning ratio \cite{sunsimple}.
Second, explicitly removing entire components in structured pruning generally leads to larger accuracy drops than unstructured pruning at the same pruning ratio \cite{sunsimple}.

Since structured pruning inevitably leads to performance degradation, previous methods \cite{han2024parameter,hu2021lora,karimi2021compacter} often rely on fine-tuning to recover model performance.
However, the fine-tuning process also faces two issues when applied to resource-constrained devices.
One of them is still the memory overhead.
A backward pass requires at least $2 \times$ the memory consumption of a forward pass, while popular stateful optimizers like AdamW \cite{loshchilovdecoupled} need at least $3 \times$.
Still taking the pruning of the 7B model as an illustration, LoRAPrune \cite{zhang2024loraprune} requires alternating with fine-tuning, resulting in a memory overhead of 18GB, which is still unacceptable for most weak devices.
Despite the memory consumption problem, fine-tuning also requires intensive large amounts of training data.
A common fine-tuning process requires approximately 50k data samples \cite{ma2023llmpruner}.
Therefore, fine-tuning is typically conducted on cloud servers.
However, when dealing with private information, \eg, medical \cite{wiest2024privacy} or financial data \cite{paul2023optimizing}, performing fine-tuning on cloud servers will raise substantial privacy concerns.
Moreover, limited device capabilities and scarce data often make device fine-tuning of LLMs on local devices impractical \cite{wu2024fedbiot}.
Therefore, it is quite necessary to develop a lightweight structured pruning method that eliminates the need for fine-tuning.

In order to avoid additional fine-tuning, post-training methods have been receiving increasing attention.
Such methods do not rely on fine-tuning the model to ensure the performance of the pruned model, effectively mitigating the issues of high memory overhead and large data requirements.
However, post-training methods always face the problem of limited general applicability.
First, the diversity of LLMs restricts the applicability of certain pruning methods to specific model designs. 
The primary differences between various LLMs lie in what activation functions they use, and what layer-internal structures they are.
For instance, Dejavu \cite{liu2023deja} is only suitable for models with ReLU activation functions.
It does not work for mainstream LLaMA models \cite{touvron2023llama}.
Second, some methods demand extensive modifications to accommodate various architectures.
SliceGPT \cite{ashkboos2024slicegpt} needs to design an adapter for each type of model before pruning because of different structures, 
thereby limiting its versatility.

To address these challenges, we propose a matrix condition-based post-training structured pruning method, called COMP.
For ease of description, we refer to the linear layer as \textit{dense} and the model layer as \textit{layer} to avoid confusion.
COMP employs a hybrid-granularity structured pruning (\ie, layer-grained and neuron-grained ) strategy.
It begins by evaluating the importance of each layer, performing layer-grained pruning, and determining the pruning ratios for the remaining layers individually. 
Next, COMP assesses the importance of neurons based on the matrix condition, and further prunes denses in each remaining layer by performing neuron-grained pruning.
Inspired by \cite{kwon2022fast}, we employ \textit{mask tuning} to restore the performance of pruned models. 
Unlike the previous approach, we specifically focus on tuning the dense mask, rather than the attention head mask or the feed-forward network mask.
%\textit{Mask tuning} adjusts the input mask of the pruned model by solving a least squares problem, ensuring that the output of each module in the pruned model remains consistent with the original model.
%This process can be completed with very little amount of data.

Our method has two advantages, and the first is low memory consumption.
When evaluating layer importance, we load layers dynamically so that a single layer is loaded at a time.
When evaluating neuron importance, we focus on neurons within a single dense, thus circumventing the need to compute global gradients.
%thus alleviating the high memory consumption by circumventing the need to compute global gradients.
The second is wide general applicability.
The entire pruning process remains agnostic to layer-internal structures and activation functions, facilitating straightforward adaptation to diverse architectures.
However, as different denses can vary substantially in function and pruning tolerance, when performing neuron-grained pruning, determining the appropriate number of pruning neurons of each dense while keeping their performance is a challenging task.

In summary, our main contributions are as follows:
% \begin{itemize}[itemsep=2pt]
\begin{itemize}[itemsep=0pt]
\item We introduce COMP, a novel post-training structured pruning method.
It efficiently prunes the model at layer-grained pruning and neuron-grained pruning and can handle LLMs of various structures with low memory consumption.
\item We propose a key evaluation metric for determining the importance of neurons. 
Building upon the metric, we design an iterative pruning method to automatically determine the number of pruning neurons in each dense, and perform mask tuning, ensuring the dense output remains effectively unchanged after pruning.
\item %The extensive experiments are conducted on A6000(48GB) to evaluate the performance of COMP on three types of large models (\ie, LLaMA2, OPT, ChatGLM3). 
% Compared to baseline methods, COMP achieves the best performance at different pruning ratios.
We conduct extensive experiments on LLMs of 3 different structures.
Experimental results indicate that COMP can prune the LLaMA-2-7B model with the requirements of only 8GB while retaining approximately 91.2\% of the average performance for downstream tasks at a 20\% pruning ratio. %给出其相比于baselines在精度和显存上的表现
\end{itemize}

==> contents/backup/motivation_backup.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[height=3.6cm]{contents/image/LLaMA-2-7BLR.pdf}
        \caption{LLaMA-2-7B}
        \label{fig:LayerRedundancy1}
    \end{subfigure}
    \hspace{0.01\linewidth}
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[height=3.6cm]{contents/image/OPT-6.7BLR.pdf}
        \caption{OPT-6.7B}
        \label{fig:LayerRedundancy2}
    \end{subfigure}
    \caption{Layer redundancy of different models. Bars with deeper color correspond to layers of higher importance.}
\label{fig:LayerRedundancy}
\vskip -0.2in
\end{figure}

Since the computational cost of backpropagation for large models is too high for typical devices, we should find another good evaluation metric for the importance of the module. 
To achieve the structural generality of the method, we design two evaluation metrics: layer importance and neuron importance within the linear layers.

\textbf{Layer Importance.}
In structured pruning, the simplest approach is directly removing the total layer.
Intuitively, if an LLM's layer has high redundancy (i.e., the inputs and outputs of that layer are very similar), then skipping that layer during inference would not significantly impact the final result.
Based on \cite{men2024shortgpt}, we define the importance of the $l$-th layer as Eq. \eqref{layerimp}:
\begin{equation}\label{layerimp}
I_l = 1 - E_{t}\Bigl[\frac{(X^l_{t})^TX^{l+1}_t}{||X^{l}_t||_2||X^{l+1}_t||_2}\Bigr]
\end{equation}
where the second term is layer redundancy, $X^l$ and $X^{l+1}$ represent the input and output of the $l$-th layer respectively, and $X^{l}_t$ means the $t^th$ row of $X^l$. 
We tested the layer redundancy in three different models and the results are shown in Figure \ref{fig:LayerRedundancy}(a) and Figure \ref{fig:LayerRedundancy}(b). 
Obviously that most of layers in the model exhibit high redundancy.
This inspires us that directly removing some layers of the model may have little impact on its performance.
We will also demonstrate this point in subsequent experiments.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Neuron Importance.}
\label{sec:Neuron Importance}
Observing that the bias term has no effect in Eq. \eqref{maskTuning}, we can further express it as:
\begin{equation}\label{lsq}
\hat{m}^{\ast}_c = \mathop{\arg\min}\limits_{\hat{m}_c} \bigl\|(m_c\circ \hat{X}^{l,k})W^{l,k}\circ \hat{m}_c - X^{l,k}W^{l,k}\bigr\|_2^2
\end{equation}
According to \cite{kwon2022fast}, Eq. \eqref{lsq} can be reformulated as a least-square problem.
For simplicity, we define a new matrix operation $F$.
Assuming $G,H \in \mathbb{R}^{p \times q}$:
\begin{align}\label{newop}
F(G,H) = u = [u_1, u_2, \cdots, u_p]^T, u_i = \sum^{q}_{j} (G \circ H)_{ij}
\end{align}
Then we can calculate $\hat{m}^{\ast}_c$ by solving:
\begin{align}\label{lsq1}
\hat{A}\hat{m}_c &= F\bigl((m_c\circ \hat{X}^{l,k})^T, W^{l,k}(X^{l,k}W^{l,k})^T\bigr)
\end{align}
where
\begin{align}\label{lsq2}
\hat{A} &= \bigl[W^{l,k}(W^{l,k})^T\bigr]\circ \bigl[(m_c\circ \hat{X}^{l,k})^T(m_c\circ \hat{X}^{l,k})\bigr]
\end{align}
Since Eq. \eqref{lsq1} is related to a linear equation, we naturally focus on the properties of the coefficient matrix $\hat{A}$.
For linear equation systems, the condition number is a commonly used metric to assess the properties of the coefficient matrix, the condition number of a matrix $Q$ is defined as follows:
\begin{equation}\label{condA}
\kappa(Q)_a = ||Q||_a \cdot ||Q^{-1}||_a
\end{equation}
where $||\cdot||_a$ is a certain matrix norm. 
$\kappa(Q)_a$ actually indicates the sensitivity of the computation involving matrix $Q$ to errors.
Since the matrix 1-norm and infinity-norm depend only on the rows or columns of the matrix, whereas the 2-norm better reflects the overall variation of the matrix and has a continuous gradient, we accordingly choose $a=2$.

We hope that the pruned model can still handle most tasks effectively, meaning that the solution 
$\hat{m}_c$ can minimize the optimization objective in most cases. 
In other words, we aim to minimize the impact of changes in $\hat{X}^{l,k}$ on the solution $\hat{m}_c$, since $X^{l,k}$ and $W^{l,k}$ are constant.
So we should make the condition number as small as possible to avoid the matrix $\hat{A}$ from becoming ill-conditioned.

Note that we can approximate $\kappa(\hat{A})_2$ by the first-order of Taylor expansion:
\begin{align}\label{condA}
\kappa(\hat{A})_2 &\approx \kappa(A)_2 + \frac{\partial \kappa(A)_2}{\partial A}(\hat{A} - A) \nonumber \\
&\approx \kappa(A)_2 - \sum^{i \in C}_{i} \sum^{q^{l,k}}_{j} W^{l,k}_{i,j} \cdot \frac{\partial \kappa(A)_2}{\partial W^{l,k}_{j,i}}
\end{align}
where $C$ is the pruned neuron set corresponding to $m^{l,k}_c$, and $A$ is the initial coefficient matrix before pruning.
So we can define the importance of $f$-th neuron in certain linear layer as follows:
\begin{align}\label{neuronimp}
    \widetilde{I}_f &= - \sum^{q^{l,k}}_{j} W^{l,k}_{j,f} \cdot \frac {\partial \kappa(A)_2}{\partial W^{l,k}_{j,f}}\nonumber \\
    &= - \sum^{q^{l,k}}_{j} W^{l,k}_{j,f} \cdot \frac {\partial \kappa(\bigl[W^{l,k}(W^{l,k})^T\bigr]\circ \bigl[(\hat{X}^{l,k})^T\hat{X}^{l,k}\bigr])_2}{\partial W^{l,k}_{j,f}}
\end{align}
As in Eq. \eqref{condA}, pruning neurons with higher $\widetilde{I}_f$ will show a more obvious increment in the $\kappa(A)_2$, which makes the solution $\hat{m}^{\ast}_c$ more sensitive to input $X^{l,k}$, leading to instability.

\begin{figure}[t]
\centering
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[height=3.6cm]{contents/image/ppl_prune_LLaMA-2-7B.pdf}
\caption{LLaMA-2-7B}
\label{fig:PPL_Pruneratio1}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[height=3.6cm]{contents/image/ppl_prune_OPT-6.7B.pdf}
\caption{OPT-6.7B}
\label{fig:PPL_Pruneratio2}
\end{subfigure}
% \vspace{-3mm}
\caption{Perplexity on Wikitext2 of models pruned with different strategies given different pruning ratios.}
\label{fig:PPL_Pruneratio}
\end{figure}

To validate the rationality of the proposed metric, we compared it with several common indicators for measuring neuron importance. 
We conducted tests on three different models based on three different pruning strategies:
\begin{itemize}
    \item Layer only: remove layers from the model in order based on $I_l$.
    \item Neuron only: remove same number of neurons from each linear layer based on $\widetilde{I}_f$.
    \item Mix: remove 2 layers from the model in order based on $I_l$, then remove the same number of neurons from rest linear layers based on $\widetilde{I}_f$.
\end{itemize}

\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.85\textwidth]{contents/image/overview.pdf}
	\caption{COMP pruning process.}
	\label{fig:overview}
\end{figure*}
As shown in Figure \ref{fig:PPL_Pruneratio}(a) and Figure \ref{fig:PPL_Pruneratio}(b), when removing a small number of layers, the change in model performance is not significant, so directly removing some layers is feasible, but simply using the method of removing layers results in a significant decrease in performance after reaching a certain pruning ratio, and it is difficult to control the actual pruning ratio. 
The method of simply removing neurons also performs poorly at high pruning ratios, it is not appropriate to subtract the same number from each linear layer due to their different importance. 
Since the Mix method combines the advantages of both, it demonstrated the best performance across all three models at the same pruning rate.
Because $\widetilde{I}_f$ only involves the parameters of a specific linear layer during computation, the memory resources required are significantly lower compared to  backpropagation across the entire model, typically requiring less memory than what is needed for deploying the model.
Moreover, because we only need to consider a linear layer during pruning, we can employ a method of dynamically loading layers, only loading one model layer into memory at a time. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Based on the above observation, we introduce two comprehensive metric for layer and neuron individually. 
Both calculations are simple and memory-efficient, making them very suitable for model pruning on general devices. 
Since the mix method performs best but still rough, in the subsequent algorithm design, we considered the problem of deciding the number of pruning parameters in different linear layers, and designed a pruning algorithm in detail. 
In the following sections, we will further discuss the specific pruning process.


==> contents/backup/prelim_backup.tex <==
% \subsection{Related Works}
% To reduce the inference cost of LLMs and increase their practical applications, model pruning has been widely used to compress large language models, which can be classified into three categories: Unstructured pruning, Semi-structured pruning, and Structured pruning:

% \textbf{Unstructured pruning} Unstructured pruning removes individual weights without considering the network's architecture. It involves pruning weights that are considered least important based on a specific criterion, such as magnitude or gradient\cite{han2015learning, frankle2018lottery, frankle2019stabilizing}.
% Unstructured pruning doesn't always lead to computational speedup because the irregular sparsity requires special hardware support (\eg, sparse matrix operations).

% \textbf{Semi-structured pruning} Semi-structured pruning compresses the model by removing M parameters within a continuous group of N parameters, which is called N:M constraint sparsity(Mishra et al., 2021).
% For instance, a 2:4 constraint ratio results in 50\% sparsity, effectively doubling the model’s inference speed when utilizing the NVIDIA Ampere GPU architecture.
% SparseGPT\cite{frantar2023sparsegpt} and RIA\cite{zhang2024plug} can both maintain the model's performance at high semi-structured sparsity (50\%) ratios without the need for retraining.
% However, semi-structured pruning still requires specific hardware support to accelerate inference.

% \textbf{Structured pruning} Structured pruning compresses LLMs by removing entire neurons, which directly reduces the dimensionality of the parameter matrix, allowing for inference acceleration without the need for specific hardware support. 	In comparison to semi-structured pruning methods, models pruned with structured pruning tend to experience a significant drop in performance under the same sparsity ratio, which typically requires fine-tuning after pruning to restore the model's performance, such as LoRAPrune\cite{zhang2024loraprune}. 
% Currently, few methods exist for structured pruning of large models that do not require fine-tuning, and each has its limitations: LLM-pruner\cite{ma2023llmpruner} requires backpropagation across the entire model to calculate group importance, resulting in high memory overhead; SliceGPT\cite{ashkboos2024slicegpt} requires more homogenous data to reduce the dimensionality of the parameter matrix, making it highly data-dependent; Dejavu\cite{liu2023deja}, while not requiring model retraining, needs to retrain the mask and is only suitable for models with ReLU activation functions (such as OPT); Bonsai\cite{dery2024everybody} searches for the optimal substructure of the model to obtain a compressed version, but it requires 40 hours to prune a 7B model, and this time increases exponentially with the model's parameter size.

\subsection{Related Works}

Model pruning has become a widely adopted technique for reducing inference costs and memory usage in LLMs.
% , thereby enhancing their practical applicability. 
% \rednote{Pruning methods can be broadly categorized into three primary strategies: unstructured, semi-structured, and structured pruning.}%这里重点就介绍structured pruning的工作，主要是一般基于梯度等的工作，和post-training的工作。unstructured, semi-structured的可以不介绍。或者开头就先说明unstructured, semi-structured的缺点，然后说明我们接下来主要介绍structured pruning的相关工作。
Herein, we focus on structured pruning for deploying LLMs on resource-constrained devices considering its inherent hardware-friendly nature and applicability, and review some related works.

% \textbf{Unstructured pruning} removes individual weights without regard to model architecture. Typical methods identify and prune weights deemed least important based on certain criteria (\ie, magnitude or gradient) \cite{han2015learning, frankle2018lottery, frankle2019stabilizing}. 
% Although unstructured pruning can effectively reduce model size, it does not always accelerate inference in practice because the induced irregular sparsity in weight matrices often requires specialized hardware (\ie, sparse matrix operations) for speedup.

% \textbf{Semi-structured pruning} enforces a more regular sparsity pattern compared to unstructured pruning. 
% Particularly, the N:M sparsity scheme, \ie, removing $M$ out of every $N$ weights in a contiguous block, has shown predictable performance gains \cite{mishra2021accelerating}. 
% For instance, a 2:4 scheme yields 50\% sparsity and doubles inference speed on NVIDIA Ampere GPUs. 
% Recent works, including SparseGPT \cite{frantar2023sparsegpt} and RIA \cite{zhang2024plug}, have demonstrated that models can preserve relatively high performance at 50\% semi-structured sparsity without retraining or fine-tuning. 
% Nonetheless, specialized hardware support remains crucial to fully leverage the speedups offered by semi-structured pruning.

% \textbf{Structured pruning} removes entire neurons (or filters), which effectively reduces the dimensionality of the weight matrices. 
% Unlike unstructured and semi-structured pruning, structured pruning can directly accelerate inference on standard hardware without specialized support. 
% However, because each pruned neuron corresponds to a complete column (or row) of the weight matrix, structured pruning often causes more severe performance drops at equivalent sparsity levels. 
% As a result, fine-tuning is usually required to recover accuracy; examples include LoRAPrune \cite{zhang2024loraprune}. 

% Despite its potential, structured pruning of LLMs without fine-tuning remains relatively underexplored, and existing methods have various limitations. 
% LLM-Pruner \cite{ma2023llmpruner} requires full-model backpropagation to compute group importance, resulting in high memory costs. 
% SliceGPT \cite{ashkboos2024slicegpt} relies on principal component analysis (PCA) to compute orthogonal matrices, which requires a large amount of calibration data.
% Dejavu \cite{liu2023deja} avoids model fine-tuning but needs to retrain the mask and is only suitable for models with ReLU activations (\ie, OPT). 
% Bonsai \cite{dery2024everybody} searches for an optimal substructure of the model to obtain a compressed version, but pruning a 7B model still takes roughly 40 hours, and the pruning time grows exponentially with model size.

Structured pruning removes entire neurons (or filters), thereby reducing the dimensions of the weight matrices in a way that directly accelerates inference on standard hardware, unlike unstructured and semi-structured pruning. 
However, because each pruned neuron corresponds to a complete column (or row) of a weight matrix, structured pruning often causes more severe performance degradation at equivalent sparsity levels, necessitating fine-tuning to restore accuracy, \ie, LoRAPrune \cite{zhang2024loraprune}.
\redcomment{Introduce more works about fine-tuning after structured pruning, and expose some shortcomings here.}

Despite its potential, applying structured pruning to LLMs without fine-tuning remains underexplored, with current methods facing several drawbacks. 
LLM-Pruner \cite{ma2023llmpruner} demands full-model backpropagation to estimate group importance, leading to substantial memory overhead. 
SliceGPT \cite{ashkboos2024slicegpt} uses principal component analysis (PCA) to form orthogonal matrices, requiring large amounts of calibration data. 
Dejavu \cite{liu2023deja} obviates the need for fine-tuning but requires retraining of the pruning mask and is restricted to models with ReLU activations (\ie, OPT). 
Bonsai \cite{dery2024everybody} searches for an optimal model substructure but takes roughly 40 hours to prune a 7B model, with computational cost growing exponentially for larger models.
\redcomment{Give a overall discussion here.}

% Herein, we focus on structured pruning for deploying LLMs on resource-constrained devices considering its inherent hardware-friendly nature and applicability.

% \subsection{Preliminaries}
% We consider an LLM built on the transformer architecture, consisting of $L$ identical layers. 
% Each layer containing a multi-head attention(MHA) layer and an FFN layer, which can also be seen as $K$ distinct linear layers.
% The parameters of the $k$-th linear layer in the $l$-th layer has an input dimension of $n^{l,k}_1$ and an output dimension of $n^{l,k}_2$, its parameters consist of the weights $W^{l,k} \in R^{n^{l,k}_1 \times n^{l,k}_2}$ and the bias $b^{l,k} \in R^{n^{l,k}_1 \times 1}$.

% \textbf{Structured pruning.} 
% Our method performs pruning on the filters within the scope of a linear layer and uses an input mask to represent the pruning process.
% Pruning the $j$-th input neuron of a linear layer, which means pruning the 
% $j$-th column of $W^{l,k}$, is equivalent to setting all the parameters in the $j$-th column to zero, \ie, $W^{l,k}_{:,j} = \mathbf{0}$. 
% If the input to the linear layer is $x^{l,k}$, this corresponds to ignoring the $j$-th dimension of 
% $x^{l,k}$.
% Assuming the number of pruned neurons is $c$, the output of the pruned linear layer can be expressed as Equation \eqref{mask}:
% \begin{eqnarray}\label{mask}
% linear(x^{l,k}; m^{l,k}_c) = W^{l,k}(m^{l,k}_c \circ x^{l,k}) + b^{l,k}
% \end{eqnarray}
% where $m^{l,k}_c \in \{0, 1\}^{n^{l,k}_1}$ is the input mask, $c$ elements of which are set to zero.

% \textbf{Mask tuning.}
% To ensure that the post-traning pruning method is effective, a training-free optimization method are crucial. 
% \cite{kwon2022fast} provides a great idea through tuning mask, which reconstruct the output activation of the original model with the remaining neurons in the pruned model, from the first to the last layer. 
% Mask tuning minimizes the changes in layer outputs before and after pruning by solving a least squares problem using a small amount of sample data, which can be formally written as Equation \eqref{maskTuning}:
% \begin{eqnarray}\label{maskTuning}
% \mathop{\arg\min}\limits_{m^{l,k}_c} ||linear(x^{l,k};m^{l,k}_c) - linear(\hat{x}^{l,k};\mathbf{1})||_2^2
% \end{eqnarray}
% where $\hat{x}^{l,k}$ is the input to the linear layer of the original model.


\subsection{Preliminaries}
We consider an LLM built on the transformer architecture, consisting of $L$ identical layers. Each layer comprises a multi-head attention (MHA) module and a feed-forward network (FFN), which can be viewed as $K$ distinct linear layers.
% As shown in Figure \ref{fig:LLM Structure}, 
For instance, LLaMA-2-7B has 32 layers, each contains 4 linear layers in MHA module and 3 linear layers in FFN module.
Let the $k$-th linear layer in the $l$-th Transformer layer have input dimension $p^{l,k}$ and output dimension $q^{l,k}$. 
Its parameters consist of a weight matrix $W^{l,k} \in \mathbb{R}^{p^{l,k} \times q^{l,k}}$ and a bias vector $b^{l,k} \in \mathbb{R}^{q^{l,k}}$.

In this work, we employ \emph{structured pruning} to compress LLMs.
However, structured pruning inevitably changes each layer’s output distribution, which significantly degrades model accuracy if no additional measures are taken.
To address this, we adopt a \emph{mask tuning} mechanism, which compensates for the performance loss induced by structured pruning. 
Assuming $T$ calibration data samples are available, each with a length of $E$ tokens, let $X^{l,k}, \hat{X}^{l,k} \in \mathbb{R}^{T \cdot E \times p^{l,k}}$ represent the inputs to the linear layer in original (unpruned) model and pruned model individually.

\textbf{Structured pruning.}
Specifically, pruning the $j$-th input neuron of a linear layer amounts to removing the $j$-th column of $W^{l,k}$ by setting it to zero, \ie, $W^{l,k}_{:,j} = \mathbf{0}$. 
This pruning corresponds to ignoring the $j$-th dimension of the linear layer's input $X^{l,k}$.
Assuming $c$ neurons are pruned, the output of the pruned linear layer can be expressed as
\begin{equation}\label{mask}
\mathrm{linear}(\hat{X}^{l,k}; m_c) = \bigl(m_c \circ \hat{X}^{l,k}\bigr)W^{l,k} + b^{l,k}
\end{equation}
where $m_c \in \{0,1\}^{p^{l,k}}$ is the input mask, and exactly $c$ entries in $m^{l,k}_c$ are set to zero.

\textbf{Mask tuning.}
To ensure the effectiveness of post-training pruning, pruned model's parameters should be slightly adjusted. 
We choose to use \textit{mask tuning}\cite{kwon2022fast}, which reconstructs the original model's output activations using the retained neurons in the pruned model from the first layer to the last. 
Mask tuning reduces the discrepancy in layer outputs before and after pruning by solving a least squares problem on a small set of samples, formally written as
\begin{equation}\label{maskTuning}
\hat{m}^{\ast}_c = \mathop{\arg\min}\limits_{\hat{m}_c} \bigl\| \mathrm{linear}(m_c \circ \hat{X}^{l,k};\hat{m}_c) - \mathrm{linear}(X^{l,k};\mathbf{1}) \bigr\|_2^2
\end{equation}
where $\hat{m}_c$ is the tuned mask.

==> contents/motivation.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[height=3.6cm]{contents/image/LLaMA-2-7BLR.pdf}
        \caption{LLaMA-2-7B}
        \label{fig:LayerRedundancy1}
    \end{subfigure}
    \hspace{0.01\linewidth}
    \begin{subfigure}{0.23\textwidth}
        \centering
        \includegraphics[height=3.6cm]{contents/image/OPT-6.7BLR.pdf}
        \caption{OPT-6.7B}
        \label{fig:LayerRedundancy2}
    \end{subfigure}
    \caption{Layer redundancy of different models. Bars with deeper color correspond to layers of higher importance.}
\label{fig:LayerRedundancy}
\vskip -0.2in
\end{figure}

Since the computational cost of backpropagation for large models is too high for typical devices, we should find another good evaluation metric for the importance of the module. 
To achieve the structural generality of the method, we design two evaluation metrics: layer importance and neuron importance within the linear layers.

\textbf{Layer Importance.}
In structured pruning, the simplest approach is directly removing the total layer.
Intuitively, if an LLM's layer has high redundancy (i.e., the inputs and outputs of that layer are very similar), then skipping that layer during inference would not significantly impact the final result.
Based on \cite{men2024shortgpt}, we define the importance of the $l$-th layer as Eq. \eqref{layerimp}:
\begin{equation}\label{layerimp}
I_l = 1 - E_{t}\Bigl[\frac{(X^l_{t})^TX^{l+1}_t}{||X^{l}_t||_2||X^{l+1}_t||_2}\Bigr]
\end{equation}
where the second term is layer redundancy, $X^l$ and $X^{l+1}$ represent the input and output of the $l$-th layer respectively, and $X^{l}_t$ means the $t^th$ row of $X^l$. 
We tested the layer redundancy in three different models and the results are shown in Figure \ref{fig:LayerRedundancy}(a) and Figure \ref{fig:LayerRedundancy}(b). 
Obviously that most of layers in the model exhibit high redundancy.
This inspires us that directly removing some layers of the model may have little impact on its performance.
We will also demonstrate this point in subsequent experiments.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Neuron Importance.}
\label{sec:Neuron Importance}
Observing that the bias term has no effect in Eq. \eqref{maskTuning}, we can further express it as:
\begin{equation}\label{lsq}
\hat{m}^{\ast}_c = \mathop{\arg\min}\limits_{\hat{m}_c} \bigl\|(m_c\circ \hat{X}^{l,k})W^{l,k}\circ \hat{m}_c - X^{l,k}W^{l,k}\bigr\|_2^2
\end{equation}
According to \cite{kwon2022fast}, Eq. \eqref{lsq} can be reformulated as a least-square problem.
For simplicity, we define a new matrix operation $F$.
Assuming $G,H \in \mathbb{R}^{p \times q}$:
\begin{align}\label{newop}
F(G,H) = u = [u_1, u_2, \cdots, u_p]^T, u_i = \sum^{q}_{j} (G \circ H)_{ij}
\end{align}
Then we can calculate $\hat{m}^{\ast}_c$ by solving:
\begin{align}\label{lsq1}
\hat{A}\hat{m}_c &= F\bigl((m_c\circ \hat{X}^{l,k})^T, W^{l,k}(X^{l,k}W^{l,k})^T\bigr)
\end{align}
where
\begin{align}\label{lsq2}
\hat{A} &= \bigl[W^{l,k}(W^{l,k})^T\bigr]\circ \bigl[(m_c\circ \hat{X}^{l,k})^T(m_c\circ \hat{X}^{l,k})\bigr]
\end{align}
Since Eq. \eqref{lsq1} is related to a linear equation, we naturally focus on the properties of the coefficient matrix $\hat{A}$.
For linear equation systems, the condition number is a commonly used metric to assess the properties of the coefficient matrix, the condition number of a matrix $Q$ is defined as follows:
\begin{equation}\label{condA}
\kappa(Q)_a = ||Q||_a \cdot ||Q^{-1}||_a
\end{equation}
where $||\cdot||_a$ is a certain matrix norm. 
$\kappa(Q)_a$ actually indicates the sensitivity of the computation involving matrix $Q$ to errors.
Since the matrix 1-norm and infinity-norm depend only on the rows or columns of the matrix, whereas the 2-norm better reflects the overall variation of the matrix and has a continuous gradient, we accordingly choose $a=2$.

We hope that the pruned model can still handle most tasks effectively, meaning that the solution 
$\hat{m}_c$ can minimize the optimization objective in most cases. 
In other words, we aim to minimize the impact of changes in $\hat{X}^{l,k}$ on the solution $\hat{m}_c$, since $X^{l,k}$ and $W^{l,k}$ are constant.
So we should make the condition number as small as possible to avoid the matrix $\hat{A}$ from becoming ill-conditioned.

Note that we can approximate $\kappa(\hat{A})_2$ by the first-order of Taylor expansion:
\begin{align}\label{condA}
\kappa(\hat{A})_2 &\approx \kappa(A)_2 + \frac{\partial \kappa(A)_2}{\partial A}(\hat{A} - A) \nonumber \\
&\approx \kappa(A)_2 - \sum^{i \in C}_{i} \sum^{q^{l,k}}_{j} W^{l,k}_{i,j} \cdot \frac{\partial \kappa(A)_2}{\partial W^{l,k}_{j,i}}
\end{align}
where $C$ is the pruned neuron set corresponding to $m^{l,k}_c$, and $A$ is the initial coefficient matrix before pruning.
So we can define the importance of $f$-th neuron in certain linear layer as follows:
\begin{align}\label{neuronimp}
    \widetilde{I}_f &= - \sum^{q^{l,k}}_{j} W^{l,k}_{j,f} \cdot \frac {\partial \kappa(A)_2}{\partial W^{l,k}_{j,f}}\nonumber \\
    &= - \sum^{q^{l,k}}_{j} W^{l,k}_{j,f} \cdot \frac {\partial \kappa(\bigl[W^{l,k}(W^{l,k})^T\bigr]\circ \bigl[(\hat{X}^{l,k})^T\hat{X}^{l,k}\bigr])_2}{\partial W^{l,k}_{j,f}}
\end{align}
As in Eq. \eqref{condA}, pruning neurons with higher $\widetilde{I}_f$ will show a more obvious increment in the $\kappa(A)_2$, which makes the solution $\hat{m}^{\ast}_c$ more sensitive to input $X^{l,k}$, leading to instability.

\begin{figure}[t]
\centering
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[height=3.6cm]{contents/image/ppl_prune_LLaMA-2-7B.pdf}
\caption{LLaMA-2-7B}
\label{fig:PPL_Pruneratio1}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
\centering
\includegraphics[height=3.6cm]{contents/image/ppl_prune_OPT-6.7B.pdf}
\caption{OPT-6.7B}
\label{fig:PPL_Pruneratio2}
\end{subfigure}
% \vspace{-3mm}
\caption{Perplexity on Wikitext2 of models pruned with different strategies given different pruning ratios.}
\label{fig:PPL_Pruneratio}
\end{figure}

To validate the rationality of the proposed metric, we compared it with several common indicators for measuring neuron importance. 
We conducted tests on three different models based on three different pruning strategies:
\begin{itemize}
    \item Layer only: remove layers from the model in order based on $I_l$.
    \item Neuron only: remove same number of neurons from each linear layer based on $\widetilde{I}_f$.
    \item Mix: remove 2 layers from the model in order based on $I_l$, then remove the same number of neurons from rest linear layers based on $\widetilde{I}_f$.
\end{itemize}

As shown in Figure \ref{fig:PPL_Pruneratio}(a) and Figure \ref{fig:PPL_Pruneratio}(b), when removing a small number of layers, the change in model performance is not significant, so directly removing some layers is feasible, but simply using the method of removing layers results in a significant decrease in performance after reaching a certain pruning ratio, and it is difficult to control the actual pruning ratio. 
The method of simply removing neurons also performs poorly at high pruning ratios, it is not appropriate to subtract the same number from each linear layer due to their different importance. 
Since the Mix method combines the advantages of both, it demonstrated the best performance across all three models at the same pruning rate.
Because $\widetilde{I}_f$ only involves the parameters of a specific linear layer during computation, the memory resources required are significantly lower compared to  backpropagation across the entire model, typically requiring less memory than what is needed for deploying the model.
Moreover, because we only need to consider a linear layer during pruning, we can employ a method of dynamically loading layers, only loading one model layer into memory at a time. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{contents/image/overview.pdf}
\caption{Illustration of the pruning process of COMP.}
\label{fig:overview}
\end{figure*}

Based on the above observation, we introduce two comprehensive metric for layer and neuron individually. 
Both calculations are simple and memory-efficient, making them very suitable for model pruning on general devices. 
Since the mix method performs best but still rough, in the subsequent algorithm design, we considered the problem of deciding the number of pruning parameters in different linear layers, and designed a pruning algorithm in detail. 
In the following sections, we will further discuss the specific pruning process.

